C*: Unifying Programming and Verification in C

Ensuring the correct functionality of systems software, given its safety-critical and low-level nature, is a primary focus in formal verification research and applications. Despite advances in verification tooling, conventional programmers are rarely involved in the verification of their own code, resulting in higher development and maintenance costs for verified software. A key barrier to programmer participation in verification practices is the disconnect of environments and paradigms between programming and verification practices, which limits accessibility and real-time verification. We introduce C*, a proof-integrated language design for C programming. C* extends C with verification capabilities, powered by a symbolic execution engine and an LCF-style proof kernel. It enables real-time verification by allowing programmers to embed proof-code blocks alongside implementation code, facilitating interactive updates to the current proof state. Its expressive and extensible proof support allows users to build reusable libraries of logical definitions, theorems, and programmable proof automation. Crucially, C* unifies implementation and proof code development by using C as the common language. We implemented a prototype of C* and evaluated it on a representative benchmark of small C programs and a challenging real-world case study: the attach function of pKVM's buddy allocator. Our results demonstrate that C* supports the verification of a broad subset of C programming idioms and effectively handles complex reasoning tasks in real-world scenarios.

==> background.tex <==
\section{Background}
\label{sec:background}

As mentioned in \cref{sec:introduction},
\cstar{} integrates two well-established techniques from program verification and theorem proving, respectively: (i) symbolic execution with separation-logic assertions, and (ii) the LCF approach for implementing theorem provers within a programming environment.
%
This section provides a brief review of them and prepares the reader for the guided tour of \cstar{} in \cref{sec:overview}.

\subsection{Separation-Logic-based Symbolic Execution}
% Proofs of low-level programs (Proving programs)



In \cstar{}, we apply an external separation-logic engine for the C language, which takes an annotated C program that has at least one assertion in each loop in the control-flow graph of the program, and produces proof obligations in the form of \emph{separation-logic entailments}.
%

\subsection{LCF-Style Theorem Proving}
% Programming proofs (Programming proofs)

What distinguishes LCF-style theorem provers is their \emph{extensibility} and \emph{programmability}.
%
Like a GUI library that provides specialized tools for building graphical interfaces, an LCF prover library offers the essential building blocks for constructing formal proofs.
%
This design allows users to define and build complex, derived inference rules and proof search routines using the full power of the programming language.
%
To ensure the soundness of the proofs, type abstraction of the theorem values must be enforced (by the meta-language type system in the LCF tradition), guaranteeing only valid formal derivations can be constructed.

In the implementation of \cstar{}, we reuse the LCF kernel of the HOL Light proof assistant~\cite{DBLP:conf/tphol/Harrison09a}, a minimal implementation of higher-order logic in OCaml.
%
We provide a first-order interface to manipulate the logic terms, theorems, and conversions in C (detailed in \cref{sec:design}).
%
This avoids the need to build a new LCF-style kernel from scratch in C, while leveraging the extensive libraries available in HOL Light for mathematical reasoning.
%




% Its characterizing features include a small trusted kernel and a mechanism to do backward reasoning with tactics and subgoaling.
%We are mostly interested in its programmability and extensibility nature.
% Over-simplified view of the LCF-style theorem prover. Actually there is conversions, tactics, etc., but they are usually encoded using function types, assembled using higher-order functions.
% We take a data-centric approach to these types as well, providing a first-order interface to manipulate them in C.

==> proof.tex <==
\section{Proof}
\label{sec:proof}
